Enhancing Embedding Representation Stability in Recommendation Systems with Semantic ID

The exponential growth of online content has posed significant challenges to ID-based models in industrial recommendation systems, ranging from extremely high cardinality and dynamically growing ID space, to highly skewed engagement distributions, to prediction instability as a result of natural id life cycles (e.g, the birth of new IDs and retirement of old IDs). To address these issues, many systems rely on random hashing to handle the id space and control the corresponding model parameters (i.e embedding table). However, this approach introduces data pollution from multiple ids sharing the same embedding, leading to degraded model performance and embedding representation instability. This paper examines these challenges and introduces Semantic ID prefix ngram, a novel token parameterization technique that significantly improves the performance of the original Semantic ID. Semantic ID prefix ngram creates semantically meaningful collisions by hierarchically clustering items based on their content embeddings, as opposed to random assignments. Through extensive experimentation, we demonstrate that Semantic ID prefix ngram not only addresses embedding instability but also significantly improves tail id modeling, reduces overfitting, and mitigates representation shifts. We further highlight the advantages of Semantic ID prefix ngram in attention-based models that contextualize user histories, showing substantial performance improvements. We also report our experience of integrating Semantic ID into Meta production Ads Ranking system, leading to notable performance gains and enhanced prediction stability in live deployments.

==> sections/z_old__7-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Overall, we find that Semantic ID improves generalization for tail items, is NE neutral for head items, and slightly beneficial for torso items. This is the case compared to not only random hashing, but also individual embeddings, indicating that the target items in our recommendation set benefit from semantics-based knowledge sharing.

Below, we take a more detailed look at how the choice of IE, RH, or SemID representation interacts with the three challenging aspects of the recommendation item distribution, as well as on user history modeling.

\paragraph{Impression skew} Semantic ID has a smaller generalization gap (last 6 hours training period performance minus evaluation performance) compared to IE and RH on torso and tail items.

% Why doesn't SemID overfit? The alignment loss metric shows that SemID clustering regularizes torso/tail embeddings that fall into different clusters, in the sense that they are further apart than their corresponding embeddings in the IE model. (While RH embeddings are also farther apart, this is likely due to ID drifting, see below.)

\paragraph{Item cardinality} While we fit IE for illustration purposes in this paper, IE is impractical in large-scale real settings. RH and SemID are both ways of dealing with large item cardinality through clustering. The cluster analysis shows that SemID clusters are more meaningful than RH clusters for the prediction problem, with lower intra-cluster variance and higher inter-cluster pairwise distance (for small clusters).

\paragraph{ID drifting}
RH has the largest performance gap when comparing the two training periods, i.e., it performs worse on data from earlier in training. Because IE lacks this large gap, we conclude the performance gap is due to ID drifting, and that RH representations lose the ability to represent older items. SemID is able to generalize to earlier in the training period.
%This may be because some learning from the old items is preserved in the weights in addition to generalizing from more recent items, although we did not measure the two effects separately.

But is this because SemID has memorized/learned from older items or its increased generalization capability? The long retention experiment indicates that SemID benefits more from longer training. Specifically, the RH baseline obtains $-0.18\%$ NE gain when increasing the training period from 4 days to 20 days, while SemID obtains $-0.23\%$ NE gain.

\paragraph{User history modeling}
In the aggregation module, we find that models trained with Semantic ID have lower entropy, token self-attention, and padding token attention, and higher attention score on the first token in the sequence. This indicates that Semantic ID-based models place more weight on higher-signal items (e.g., the first item in the sequence, rather than padding tokens), have attention score distributions that are less diffuse over the entire sequence (e.g., lower entropy), and for Transformer, place higher weights on other tokens rather than self-attending. These metrics are a promising signal that Semantic ID item representations are more meaningful than their random hashing-based counterparts.
